Loop Dropout: Regularizing Shared Updates in Looped Language Models

Looped language models separate computational depth from parameter count by repeatedly applying the same transformer block. Adapting these models requires a shared update that remains effective as hidden states evolve throughout the recurrent computation. Our empirical analysis reveals a pronounced late-loop bias in standard low-rank adaptation (LoRA): the shared update provides limited adaptation at early loop positions. This imbalance motivates training shared updates under varying combinations of their applications. Randomly omitting adapter applications alone, however, does not improve task performance; it reduces expected update strength during training while leaving inference unchanged. We introduce Loop Dropout, which couples stochastic masking of adapter applications with inverse-survival rescaling to preserve expected update strength and promote effective adaptation across loops. Extensive experiments demonstrate improved mathematical reasoning across model sizes, adapter ranks and training recipes, with benefits extending to general instruction tuning and code generation. Loop Dropout outperforms existing LoRA variants and adapter regularizers, while further analysis shows stronger early-loop adaptation. Every backbone loop remains active, and inference applies the adapter at all loops using standard LoRA without additional trainable parameters or inference computation. Code is available at https://github.com/NUS-HPC-AI-Lab/loop-dropout.

==> figures/teaser_activation.tex <==
% !TEX root = ../main.tex
\begin{tikzpicture}[x=0.94cm,y=1cm,font=\small,text=FigInk]
\path[use as bounding box] (-0.56,-0.243) rectangle (6.48,3.843);
\foreach \loopidx/\xx in {1/1.72,2/2.77,3/3.82,4/4.87} {
  \node[font=\footnotesize] at (\xx,3.591) {Loop \loopidx};
  \node[draw=FigOutline,fill=FigNeutral,rounded corners=2pt,
        minimum width=0.74cm,minimum height=0.48cm,inner sep=0pt]
        (w\loopidx) at (\xx,3.114) {$W$};
}
\node[font=\footnotesize] (hin) at (0.70,3.114) {$h_0$};
\node[font=\footnotesize] (loss) at (6.02,3.114) {Loss};
\draw[-{Latex[length=1.4mm]},FigInk] (hin) -- (w1);
\draw[-{Latex[length=1.4mm]},FigInk] (w1) -- (w2);
\draw[-{Latex[length=1.4mm]},FigInk] (w2) -- (w3);
\draw[-{Latex[length=1.4mm]},FigInk] (w3) -- (w4);
\draw[-{Latex[length=1.4mm]},FigInk] (w4) -- (loss);
\foreach \active/\yy in \teaserrows {
  \node[anchor=east,font=\footnotesize,inner sep=1.5pt] at (1.29,\yy)
    {\teasercondition{\active}};
  \foreach \loopidx/\xx in {1/1.72,2/2.77,3/3.82,4/4.87} {
    \ifnum\loopidx=\active
      \node[fill=FigInk,draw=FigInk,text=white,rounded corners=1.5pt,
            minimum width=0.64cm,minimum height=0.38cm,inner sep=0pt]
            at (\xx,\yy) {$\Delta$};
    \else
      \node[draw=FigOutline,fill=white,text=FigInk!55,dashed,
            rounded corners=1.5pt,minimum width=0.64cm,
            minimum height=0.38cm,inner sep=0pt] at (\xx,\yy) {$0$};
    \fi
  }
}
\node[font=\footnotesize,text=FigInk!80] at (3.24,0.02)
  {All Four Backbone Loops Run};
\end{tikzpicture}


==> figures/teaser_data.tex <==
% Generated from figures/teaser.dat by build.sh; do not edit.
\pgfplotstableread[row sep=\\]{
loop lora loop_dropout\\
1 11.9417189206 30.7617953266\\
2 19.0722207766 35.1684736564\\
3 26.4861872855 35.9477552180\\
4 32.4041068412 35.6809071736\\
}\teaserdata


==> figures/teaser_reduction.tex <==
% !TEX root = ../main.tex
% Percentage loss reductions from the same frozen-model baseline.
% Read the saved data directly; match the diagram's activation conditions.
\input{figures/teaser_data.tex}
\begin{tikzpicture}[x=1cm,y=1cm,font=\footnotesize,text=FigInk]
\path[use as bounding box] (-0.45,-0.243) rectangle (5.95,3.843);
\node[font=\small] at (3.05,3.591) {Loss Reduction (\%)};
\fill[FigBase] (1.08,3.034) rectangle (1.36,3.194);
\node[anchor=west] at (1.46,3.114) {LoRA};
\fill[FigMain] (3.05,3.034) rectangle (3.33,3.194);
\node[anchor=west] at (3.43,3.114) {Loop Dropout};
\draw[FigOutline,line width=0.4pt] (1.52,0.18) -- (1.52,2.83);
\node[font=\footnotesize,text=FigInk!70] at (1.52,0.02) {0};
\foreach \loopidx/\yy in \teaserrows {
  \pgfmathtruncatemacro{\row}{\loopidx-1}
  \pgfplotstablegetelem{\row}{lora}\of\teaserdata
  \pgfmathsetmacro{\basevalue}{\pgfplotsretval}
  \pgfplotstablegetelem{\row}{loop_dropout}\of\teaserdata
  \pgfmathsetmacro{\oursvalue}{\pgfplotsretval}
  \node[anchor=east,inner sep=1.5pt] at (1.31,\yy)
    {\teasercondition{\loopidx}};
  \fill[FigBase] (1.52,\yy+0.08) rectangle ({1.52+0.10*\basevalue},\yy+0.26);
  \fill[FigMain] (1.52,\yy-0.26) rectangle ({1.52+0.10*\oursvalue},\yy-0.08);
  \node[anchor=west,inner sep=2pt] at ({1.52+0.10*\basevalue},\yy+0.17)
    {\pgfmathprintnumber[fixed,precision=1,zerofill]{\basevalue}};
  \node[anchor=west,inner sep=2pt,text=FigMain] at ({1.52+0.10*\oursvalue},\yy-0.17)
    {\pgfmathprintnumber[fixed,precision=1,zerofill]{\oursvalue}};
}
\end{tikzpicture}

